Evolving Image Compositions for Feature Representation Learning

Convolutional neural networks for visual recognition require large amounts of training samples and usually benefit from data augmentation. This paper proposes PatchMix, a data augmentation method that creates new samples by composing patches from pairs of images in a grid-like pattern. These new samples are assigned label scores that are proportional to the number of patches borrowed from each image. We then add a set of additional losses at the patch-level to regularize and to encourage good representations at both the patch and image levels. A ResNet-50 model trained on ImageNet using PatchMix exhibits superior transfer learning capabilities across a wide array of benchmarks. Although PatchMix can rely on random pairings and random grid-like patterns for mixing, we explore evolutionary search as a guiding strategy to jointly discover optimal grid-like patterns and image pairings. For this purpose, we conceive a fitness function that bypasses the need to re-train a model to evaluate each possible choice. In this way, PatchMix outperforms a base model on CIFAR-10 (+1.91), CIFAR-100 (+5.31), Tiny Imagenet (+3.52), and ImageNet (+1.16).

==> 000figures.tex <==

% \begin{figure*}[t] % [t]
% \centering
%   \includegraphics[width=.92\textwidth]{Images/FIG1_MASK_2IMGs_3.pdf}
% \caption {Overview of PatchMix. We first create a binary mask \textit{M} with \textit{P}x\textit{P} number of patches using our proposed PatchMix strategies: Guided PatchMix and its variation Random PatchMix (see Section \ref{sec:meth} for details on how to obtain the mask). This mask is then used to interpolate two random images which will create a new image sample. This generated sample is used to train the model, a CNN with the last convolutional layer modified to create \textit{P}x\textit{P} patches of equal size. In this way, we are able to output the values corresponding to the input patches corresponding to each image, and the mixed output of the whole new image. }
% \label{fig:fig_gridmix}
% %\vspace{-0.2in}
% \end{figure*}



==> 041datasummary.tex <==
\subsection{Tasks and Datasets}
We evaluate PatchMix on four different tasks : 
(1) {\bf Supervised Image Classification:} We show classification results on CIFAR~\cite{cifar10, cifar100} with ResNet-32, PreActResNet-56, PreActResNet-164 architectures~\cite{He2016DeepRL} and MobileNetv2~\cite{Sandler2018MobileNetV2IR}, an architecture notable for it's lightweight backbone. For this architecture we set the first, third, and fourth blocks' stride sizes to 1 instead of 2 in order to train CIFAR-10. We also show classification results with ResNet50 on the ImageNet ILSVRC~\cite{russakovsky2015imagenet, imagenet_cvpr09} dataset and Tiny Imagenet~\cite{tiny_imagenet_Le2015TinyIV}, a subset of ImageNet that contains 200 classes. (2) {\bf Weakly Supervised Object Localization(WSOL) and Object Detection}: We show results on the CUB-200-2011 dataset~\cite{Wah2011TheCB}, a fine-grained bird categorization task, and we show results on Pascal VOC~\cite{VOC} using Fast-RCNN.
(3) {\bf Transfer Learning}: We compare different models trained on ImageNet ILSVRC using different interpolation techniques, and show the transfer learning capabilities of each model on the CUB-200-2011, the SUN397~\cite{SUN} classification task with 397 scene categories, the fine-grained classification task of Aircraft (FGVC-Aircraft)~\cite{aircraft_maji13}, and the Food-101~\cite{food101_bossard14} dataset classification task. We also show the superior transfer learning capabilities of PatchMix on standard multi-label datasets, and the image captioning task on MS-COCO. 
(4) {\bf Robustness}:  We  show  results on robustness when attacking a model with adversarial perturbations using the Fast Gradient Sign Method (FGSM)~\cite{whiteBoxAttack43405} white box attack on the ImageNet validation set.


==> 090discussion.tex <==
\section{Discussion}

%(1) flexible spatial mix

%(2) better patch-level features 

%(3) faster search of configuration


Evolutionary search has been used in previous work for neural architecture search (NAS) where a space of possible network designs is explored, and can be extended for data augmentation where a combinatorial space of image transformations are explored. 
 In both cases, the bottleneck is to evaluate each configuration -- as it requires training a deep neural network to assess these choices. This has been bypassed in the past by perhaps training only on a smaller subset of the training data, or not training the model until convergence~i.e.~using an early stopping criteria. Our work goes beyond that as we are able to entirely bypass any amount of training. Our idea of using a PatchMix model pretrained on random configurations to define a fitness criteria allows for this to happen. We are surprised this was possible as a pretrained model that has seen arbitrary grid configurations is likely not to generalize on a fixed set of grid configurations. Our first idea was to just use this criteria as a fitness goal where new configurations are considered fit if they yield good results under the pretrained model. However, we found that on the contrary, fixed grid configurations that are challenging for the PatchMix model trained under random grid configurations are more informative and conducive to better models trained under fixed configurations. In the worst case scenario, our fitness function would be $2,000$ times faster than a fitness function that relies on training a model for $400$ epochs until convergence on the training split which is $5$ times larger than the validation set, since our fitness criteria only needs to iterate once over the validation set or a subset of the validation set.





